\textit{C. elegans} collectively forms dynamical networks

Understanding physical rules underlying collective motions requires perturbation of controllable parameters in self-propelled particles. However, controlling parameters in animals is generally not easy, which makes collective behaviours of animals elusive. Here, we report an experimental system in which a conventional model animal, \textit {Caenorhabditis elegans}, collectively forms dynamical networks of bundle-shaped aggregates. We investigate the dependence of our experimental system on various extrinsic parameters (material of substrate, ambient humidity and density of worms). Taking advantage of well-established \textit {C.~elegans} genetics, we also control the intrinsic parameters (genetically determined motility) by mutations and by forced neural activation via optogenetics. Furthermore, we develop a minimal agent-based model that reproduces the dynamical network formation and its dependence on the parameters, suggesting that the key factors are alignment of worms after collision and smooth turning. Our findings imply that the concepts of active matter physics may help us to understand biological functions of animal groups.

==> sup.tex <==
\newpage
\section*{Supplementary Information}
\subsection*{Video}
\noindent{\bf Video 1 $\mid$ Dynamical network that emerged on a glass surface.} 
The compartment size distribution shown in Fig. 4c was generated from this video. The movie is played 500 times faster than the real-time recording rate.
 
\noindent{\bf Video 2 $\mid$ Effect of humidity on worm interaction.} 
The attraction and alignment of worms were enhanced by their surrounding water and increased with increasing humidity. This video was created by cropping Supplementary Video 3 with contrast enhancement. The movie plays 100 times faster than the real-time recording rate.

\noindent{\bf Video 3 $\mid$ Dynamical network that emerged on the lid of a Petri plate.} 
Wild-type dauer worms were propagated using DFA on NGM in a Petri plate. The worms self-organized inside the lid. The humidity was changed as described in the Methods section. Images were taken from above the lid (Extended Data Fig. 1). The snapshot shown in the upper row of Fig. 2b was created from this video. The movie plays 100 times faster than the real-time recording rate.
 
\noindent{\bf Video 4 $\mid$ Running aggregates in higher humidity.} Images were taken from above the lid of a Petri plate. The humidity was varied as described in the Methods section. The movie is played 300 times faster than the real-time recording rate.

\noindent{\bf Video 5 $\mid$ Dynamical network of \textit{mec-4(e1611)} mutant.} The \textit{mec-4(e1611)} mutants were propagated in the same manner as the wild-type worms (Supplementary Video 3). The snapshot shown in the lower row of Fig. 2b was created using this video. The movie plays 100 times faster than the real-time recording rate.

\noindent{\bf Video 6 $\mid$ Optogenetics with blue light exposure for 0.5, 1.0 and 2.0 s and light intensity of approximately 165 \si{\micro\watt\per\square\milli\meter}.} 
Illumination is indicated by light blue shading. Short-term illumination (0.5 s) caused no obvious change in worm aggregation. In contrast, at 1.0 s illumination, the worms exhibited a response in which some of the worms temporarily diffused from the aggregates but returned to them. With long-term illumination (2.0 s), the aggregates were disrupted and dispersed. The bundle-shaped aggregate was stable, but the excess activation of the inactive worms caused its collapse. The movie is played 6.7 times faster than the real-time recording rate.

\noindent{\bf Video 7 $\mid$ Optogenetics with blue light exposure for approximately 30 s.} 
Long-term illumination was performed with mild light intensity (approximately 50 \si{\micro\watt\per\square\milli\meter}). Illumination is indicated by light blue shading. This activation initially caused the arborization and collapse of bundles. Finally, a network different from the initial structure was formed. The movie is played 6.7 times faster than the real-time recording rate.

\noindent{\bf Video 8 $\mid$ Optogenetics with 0.5, 1.0 and 2.0 s blue light illumination without ATR.} 
The light intensity was approximately 165 \si{\micro\watt\per\square\milli\meter}. Each illumination is indicated by light blue shading. Note that the illuminations induced no obvious change in the bundles, indicating that the response of the worms was dependent on ChR2 activity. The movie plays 6.7 times faster than the real-time recording rate.

\noindent{\bf Video 9 $\mid$ Single-worm tracking.} 
Worms exhibit circular movements on a glass surface. The trajectories indicated in Fig. 3d were created from this video. The movie is played 500 times faster than the real-time recording rate.

\noindent{\bf Video 10 $\mid$ Collective motion of the model.}  
The average density was 4 per unit length square. $k^{\rm{a}}=0.002$. Initially, $\bm{r}_i$ and $\theta_i$ were random. The colour shows the average number density during 10 time units.
 
\noindent{\bf Video 11 $\mid$ Collective motion of the model with inactive particles.} 
The average numerical density was 4 per unit length square. $k^{\rm{a}}=0.0054$. Initially, 30\% of particles were inactive. The colour shows the average number density during 10 time units. From 200 to 205 in the left movie (to 400 in the right movie), all particles were active to simulate light stimulation, indicated by light blue shading. The long stimulation led to the collapse of the network.

